XR-MBT: Multi-modal Full Body Tracking for XR through Self-Supervision with Learned Depth Point Cloud Registration

Tracking the full body motions of users in XR (AR/VR) devices is a fundamental challenge to bring a sense of authentic social presence. Due to the absence of dedicated leg sensors, currently available body tracking methods adopt a synthesis approach to generate plausible motions given a 3-point signal from the head and controller tracking. In order to enable mixed reality features, modern XR devices are capable of estimating depth information of the headset surroundings using available sensors combined with dedicated machine learning models. Such egocentric depth sensing cannot drive the body directly, as it is not registered and is incomplete due to limited field-of-view and body self-occlusions. For the first time, we propose to leverage the available depth sensing signal combined with self-supervision to learn a multi-modal pose estimation model capable of tracking full body motions in real time on XR devices. We demonstrate how current 3-point motion synthesis models can be extended to point cloud modalities using a semantic point cloud encoder network combined with a residual network for multi-modal pose estimation. These modules are trained jointly in a self-supervised way, leveraging a combination of real unregistered point clouds and simulated data obtained from motion capture. We compare our approach against several state-of-the-art systems for XR body tracking and show that our method accurately tracks a diverse range of body motions. XR-MBT tracks legs in XR for the first time, whereas traditional synthesis approaches based on partial body tracking are blind.

==> figures/point_cloud_parsing.tex <==
\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figures/images/pc_parsing.PNG}
\caption{\label{fig:point_cloud_parsiong} Example of point cloud parsing from our PC-encoder \RK{Denys todo: show the parsing for X motions}}
\end{figure}

==> figures/runtime_architecture.tex <==
\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figures/images/model_runtime_architecture.PNG}
\caption{\label{fig:runtime_archi} Runtime architecture. \RK{TOOD: optionally add transition}\MM{if we highlight which is train-time only, this fig could be merged with above}}
\end{figure}

==> figures/spc_training.tex <==
\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figures/images/SPC_model_architecture.PNG}
\caption{\label{fig:spc_training}  Point Cloud Semantic (PCS) model training procedure. This model is composed of an encoder module based on the PointNet architecture. The decoder takes as input \RK{do we use the sparse pose loss in the end. Modify to locak and global features. }}
\end{figure}

==> supmat/figures/extended_visual_pc_results_source.tex <==


\begin{figure}
\centering
\sbox0{\includegraphics{supmat/figures/images/ex1_raw.png}}%
\begin{subfigure}{.28\textwidth}
    \centering
    \includegraphics[height=4.5cm]{supmat/figures/images/ex1_img.png}  
\end{subfigure}
\begin{subfigure}{.28\textwidth}
    \centering
    \includegraphics[clip,trim={.2\wd0} 0 {.2\wd0} 0,height=4.5cm]{supmat/figures/images/ex1_raw.png}  
\end{subfigure}
\begin{subfigure}{.28\textwidth}
    \centering
    \includegraphics[clip,trim={.2\wd0} 0 {.2\wd0} 0,height=4.5cm]{supmat/figures/images/ex1_labeled.png}  
\end{subfigure}
\par
\begin{subfigure}{.28\textwidth}
    \centering
    \includegraphics[height=4.5cm]{supmat/figures/images/ex2_img.png}  
\end{subfigure}
\begin{subfigure}{.28\textwidth}
    \centering
    \includegraphics[clip,trim={.2\wd0} 0 {.2\wd0} 0,height=4.5cm]{supmat/figures/images/ex2_raw.png}  
\end{subfigure}
\begin{subfigure}{.28\textwidth}
    \centering
    \includegraphics[clip,trim={.2\wd0} 0 {.2\wd0} 0,height=4.5cm]{supmat/figures/images/ex2_filtered.png}  
\end{subfigure}
\caption{Additional point cloud labelling results.}
\label{fig:extended_visual_pc_results}
\end{figure}

==> tables/mocap.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.3mm}
\newcommand{\sz}{\hspace{1mm}}
\renewcommand{\arraystretch}{1.2}
\caption{Position Error (PE) per action labels using Mocap data and synthetic point clouds}
\begin{center}
\begin{tabular}{ l| ccccc}
\toprule
Action Label & AGROL \cite{du2023agrol} & XR-MBT & XR-MBT + SSL without learned semantics  & MBT + SSL \\
\midrule
walking  &  xx  & xxx &   xxx  & xxx  \\
kicking &  xx  & xxx &   xxx  & xxx  \\
knee strikes  &  xxx  & xxx &   xxx  & xxx  \\
football &  xcx  & xxx &   xxx  & xxx  \\
tennis &  xcx  & xxx &   xxx  & xxx  \\
lundges &  xcx  & xxx &   xxx  & xxx  \\
boxing &  xcx  & xxx &   xxx  & xxx  \\
dancing &  xcx  & xxx &   xxx  & xxx  \\

\bottomrule 
\centering

\end{tabular}
\end{center}
\label{tbl:mocap}
\end{table}


